Systematic KMTNet Planetary Anomaly Search, Paper VII: Complete Sample of $q < 10^{-4}$ Planets from the First Four-Year Survey

We present the analysis of seven microlensing planetary events with planet/host mass ratios $q < 10^{-4}$: KMT-2017-BLG-1194, KMT-2017-BLG-0428, KMT-2019-BLG-1806, KMT-2017-BLG-1003, KMT-2019-BLG-1367, OGLE-2017-BLG-1806, and KMT-2016-BLG-1105. They were identified by applying the Korea Microlensing Telescope Network (KMTNet) AnomalyFinder algorithm to 2016--2019 KMTNet events. A Bayesian analysis indicates that all the lens systems consist of a cold super-Earth orbiting an M or K dwarf. Together with 17 previously published and three that will be published elsewhere, AnomalyFinder has found a total of 27 planets that have solutions with $q < 10^{-4}$ from 2016--2019 KMTNet events, which lays the foundation for the first statistical analysis of the planetary mass-ratio function based on KMTNet data. By reviewing the 27 planets, we find that the missing planetary caustics problem in the KMTNet planetary sample has been solved by AnomalyFinder. We also find a desert of high-magnification planetary signals ($A \gtrsim 65$), and a follow-up project for KMTNet high-magnification events could detect at least two more $q < 10^{-4}$ planets per year and form an independent statistical sample.

==> draft.tex <==

\begin{table*}[htb]
    \renewcommand\arraystretch{1.25}
    \centering
    \caption{Parameters of Models without Parallax for \eventf}
    \begin{tabular}{c|c c c|c}
    \hline
    \hline
    Parameters & Close A & Close B & Wide & 1L2S \\
    \hline
    $\chi^2$/dof & $1658.5/1653$ & $1685.2/1653$ & $1670.1/1653$ & $1684.6/1653$ \\
    \hline
    $t_{0,1}$ (${\rm HJD}^{\prime}$)  & $8024.377 \pm 0.019$ & $8024.371 \pm 0.018$ & $8024.369 \pm 0.019$ & $8024.369 \pm 0.020$ \\
    $t_{0,2}$ (${\rm HJD}^{\prime}$) & ...  & ... & ... & $8003.447 \pm 0.071$ \\
    $u_{0,1}$  & $0.0219 \pm 0.0014$ & $0.0246 \pm 0.0020$ & $0.0240 \pm 0.0013$ & $0.0245 \pm 0.0018$ \\
    $u_{0,2}$ & ... & ... & ... & $0.0000 \pm 0.0018$ \\
    $\te$ (days)  & $79.0 \pm 4.5$ & $71.1 \pm 5.1$ & $72.6 \pm 3.4$ & $70.7 \pm 4.6$ \\
    $\rho_1$ ($10^{-3}$) & $1.05_{-0.25}^{+0.40}$ & $2.04_{-0.51}^{+0.59}$ & $<1.5$ & ... \\
    $\rho_2$ ($10^{-3}$) & ... & ... & ... & $<7.0$ \\
    $q_{f,I} (10^{-3})$ & ... & ... & ... & $2.89 \pm 0.76$ \\
    $\alpha$ (rad)  & $0.0605 \pm 0.0037$ & $0.1060 \pm 0.0042$ & $3.2251 \pm 0.0014$ & ... \\
    $s$ & $0.8732 \pm 0.0064$ & $0.8623 \pm 0.0091$ & $1.1642 \pm 0.0095$ & ... \\
    $\log q$ & $-4.545 \pm 0.158$ & $-4.693 \pm 0.146$ & $-4.872 \pm 0.117$ & ... \\
    $I_{\rm S, KMTC}$ & $21.26 \pm 0.07$ & $21.14 \pm 0.08$ & $21.16 \pm 0.06$ & $21.19 \pm 0.08$ \\
    \hline
    \hline
    \end{tabular}
    %\tablecomments{$\sigma(\pi_{\rm E, \parallel}) \sim 0.05$}
    \label{parm6}
\end{table*}
